Forecaster-aided User Association and Load Balancing in Multi-band Mobile Networks

Cellular networks are becoming increasingly heterogeneous with higher base station (BS) densities and ever more frequency bands, making BS selection and band assignment key decisions in terms of rate and coverage. In this paper, we decompose the mobility-aware user association task into (i) forecasting of user rate and then (ii) convex utility maximization for user association accounting for the effects of BS load and handover overheads. Using a linear combination of normalized mean-squared error and normalized discounted cumulative gain as a novel loss function, a recurrent deep neural network is trained to reliably forecast the mobile users' future rates. Based on the forecast, the controller optimizes the association decisions to maximize the service rate-based network utility using our computationally efficient (speed up of 100x versus generic convex solver) algorithm based on the Frank-Wolfe method. Using an industry-grade network simulator developed by Meta, we show that the proposed model predictive control (MPC) approach improves the 5th percentile service rate by 3.5x compared to the traditional signal strength-based association, reduces the median number of handovers by 7x compared to a handover agnostic strategy, and achieves service rates close to a genie-aided scheme. Furthermore, our model-based approach is significantly more sample-efficient (needs 100x less training data) compared to model-free reinforcement learning (RL), and generalizes well across different user drop scenarios.

==> v2/introduction_old.tex <==
\section{Introduction}
\label{Sec:Intro}
% To meet the unrelenting demand for wireless data, network operators are shifting their attention towards multi-tier and multi-band heterogeneous deployments to boost network capacity through increased spatial and spectral reuse.
Cellular networks continue to trend towards multi-tier and multi-band deployments to meet intense consumer demands for faster and more ubiquitous data connectivity.
% The use of low-power and low-cost small cell technology enables flexible deployment and helps offload traffic from the the macrocells.
The use of low-power small cell technology enables flexible deployments and helps boost network capacity through increased spatial reuse.
% Meanwhile, with more spectrum being released---such as the $3.7 - 4.2$ GHz in the ``C-band"---using multiple orthogonal frequency bands allows for larger transmission bandwidth.
Meanwhile, more spectrum is being released, for instance almost 500 MHz recently in the 3.7 - 4.2 GHz ``C-band" and more to be auctioned in the ``beachfront'' bands from 1 to 2.6 GHz.  Assigning users to bands and cells is an increasingly complicated problem, with large implications on the overall network coverage and throughput, particularly in the context of mobility.  The conventional strategy of simply maximizing \snr or \sinr for user association tends to lead to an imbalanced load distribution and can severely degrade both a given user's as well as the overall service rate \cite{Seven_Andrews13}.  Our goal in this paper is to develop an optimal band assignment and \BS selection strategy for multi-band heterogeneous networks that accounts for the bandwidth and propagation characteristics of each band, along with the traffic load,  user mobility, and handover overhead.

\subsection{Motivation, Background, and Scope of Paper}
% \red{Enabled by carrier aggregation,} a 
A multi-band deployment increases the overall bandwidth as well as number of connection options for subscribers, however, it comes at the cost of increased complexity, especially in the context of mobility \cite{andrews14overview}.
% Conventional user association---\BS selection and band assignment---policies that maximize received signal power or \sinr lead to preferential association towards the lower bands (offering better penetration and lower pathloss) and macrocells (transmitting at higher power-levels) resulting in an unbalanced load distribution across bands and \BSs \cite{Seven_Andrews13}.
Traditional \emph{user association}---meaning a user's \BS selection and band assignment---policies that maximize received signal power or \sinr lead to preferential association towards the lowest frequency bands---which offer better penetration and lower pathloss---and to tower-mounted macrocells with higher transmit power.
Such association rules are highly sub-optimal in terms of throughput, because higher carrier frequencies typically offer wider bandwidths while small cells are much more lightly loaded.
Furthermore, heterogeneous deployments with small coverage areas are more prone to frequent \hos and consequently poor service rates due to transmission delays, ping-pong effects, and connection drops \cite{Arshad_Velocity17, feriani22multiobjective}. 
%This results in an unbalanced load distribution across bands and \BSs \cite{Seven_Andrews13}, and the small cells and the higher frequency bands remain under-utilized.
% As a consequence, the small cells and the higher frequency bands---which typically offer wider bandwidths---remain under-utilized, which is highly suboptimal in terms of throughput.

As a result, there has been considerable work investigating user association and cell load balancing.
% for fair resource management. 
These include stochastic geometry studies which analytically characterize the throughput gain from load balancing \cite{singh13offloading, kassir22analysis, Modeling_Lin13} and optimization-based user association strategies \cite{shen14distributed, ye13user, kim12distributed, ye16user, liu19joint, teng21joint}.
In \cite{ye13user, shen14distributed}, authors propose log-utility-based association strategies to achieve network-wide proportional fairness for static users, and \cite{kim12distributed} presents $\alpha$-optimal load balancing strategy for inhomogeneous user traffic.
The user association problem has also been studied in conjunction with power allocation \cite{liu19joint}, massive MIMO \cite{ye16user}, and \BS activation strategies \cite{teng21joint}, under the network utility maximization framework.
Meanwhile, in actual cellular deployments, proactive load balancing is usually accomplished by biasing user association towards small cells \cite{rakotomanana16optimum, ghosh12heterogeneous} by some tunable dB value.
For example, a small cell could have a 5-10 dB \snr bias relative to a macrocell \cite{QualcommHeNets}. 

Accounting for user mobility within the optimization framework is generally intractable, with limited studies in the literature, mostly using simplistic mobility models.
% \cite{sang04coordinated, addali19dynamic}
However, a variety of studies underscore the benefits of mobility-aware user association and \ho management \cite{addali19dynamic, lin13towards, hsueh17equivalent, Arshad_Velocity17}.
The authors in \cite{lin13towards, hsueh17equivalent} characterize \ho rate as a function of user velocity and \BS density. 
By leveraging similar stochastic geometry-based analysis \cite{Arshad_Velocity17} proposes a \BS skipping \ho policy for high-speed users in a two-tier cellular network.
For a comprehensive survey of mobility models---both trace-based and probabilistic---and mobility-aware performance characterizations, please refer to \cite{tabassum19fundamentals}.

Mobility-aware user association has been considered recently as a \rl problem \cite{zhang18loadbalancing, Handover_Wang18, zhao19deep, xu19load, gupta21load, wu21load, feriani22multiobjective}.
Among these, \cite{zhao19deep, gupta21load} aim to optimize the network utility within the \rl framework, \cite{zhang18loadbalancing, Handover_Wang18} maximize the sum-rate, and \cite{xu19load, feriani22multiobjective} optimize cell individual offset parameters.
However, such model-free \rl techniques are known to be sample-inefficient \cite{mai2022sample}, and there has been a push towards scalable and sample-efficient formulations \cite{wu21load, alcaraz22model,agarwal2022taskdriven}. 
The authors in \cite{wu21load} use transfer learning and a model-based \rl solutions was explored in \cite{alcaraz22model} for load balancing and network optimization.

In this work, we focus on the most widely deployed frequency bands, namely the ``sub-6 GHz" or ``frequency range 1 (FR1)" range, which still carry vast majority of cellular traffic even in 5G deployments today, despite the introduction of millimeter wave bands.  At these lower frequencies, initial access and control channel communication can be reliably performed without the requirement for highly directional beamforming, which greatly simplifies the user association and \ho.   A key challenge for load balancing with highly directional transmissions is that the association decision for a given UE has a subsequent affect on the interference, making \sinr and load-based association decisions problematic and nonconvex.  Furthermore, since such bands will be lightly loaded for the forseeable future, it may not be necessary to perform load balancing on them.  Thus, we restrict our attention to the lower bands in this work.


% In this work, we propose a learning-based \mpc approach where a forecaster predicts the future trajectory based on past measurements, and the controller performs user association based on the forecast.
% % In this work, we propose a learning-based \mpc solution for multi-band user association. 
% The objective is to maximize the cumulative utility over a time-horizon using the forecast of the user trajectory.
% We empirically show that forecaster training is much more sample-efficient compared to a model-free \rl algorithm on a large-scale network.
% We propose a computationally efficient Frank-Wolfe algorithm for the \mpc.


\subsection{Contributions}

The overarching technical contribution of this paper is the development of a novel framework for mobility-aware \BS and frequency band association in a large-scale cellular network.  The key elements and unique aspects of our approach are summarized as follows.

% \textbf{Learning-based \mpc.}
\textbf{Optimization framework for mobility and \ho aware association.}
We formulate a novel optimization problem to maximize network utility based on the users' service rates.
In \secref{subsec:service_rate} we define the user service rate, which depends on the load on the serving \BS, the \sinr between the user and \BS, and the signaling overhead in case of a triggered \ho.
A key insight is that in a mobile network, the user association task can be decomposed into forecasting user trajectories and thus their future rates, and then a convex utility maximization problem based on those predicted rate values.
As such, we propose a learning-based \mpc approach in \secref{sec:mpc_formulation}, where we only need data-driven learning for forecasting, while we can employ interpretable utility maximization for band assignment and \BS selection.
% Thus, in \secref{sec:forecaster_design}, we design a forecaster to model and predict the users' mobility patterns.
% Then, in \secref{sec:mpc_formulation} we formulate a convex utility maximization problem which uses these trajectory predictions to solve for user associations that maximize network utility.
% accounts for the adverse effects of load imbalance and excessive \hos.

\textbf{Sample-efficient forecaster design.} 
In \secref{sec:forecaster_design}, we design a forecaster to model and predict the users' mobility patterns, which are then used by the \mpc controller to solve for associations that maximize the network utility.
The forecaster is trained in a supervised fashion, which is generally more sample-efficient and stable compared to model-free \rl.
% To further improve the sample-efficiency, instead of the task-agnostic mean-squared error loss we identify important characteristics of a forecast relevant to the utility maximization task and develop a novel loss function to train a task-aware forecaster.
To further improve the sample-efficiency, in we identify important characteristics of a ``good" forecast for the given utility maximization problem and develop a novel loss function to train a task-aware forecaster, instead of using the task-agnostic mean-squared error loss.
We compare the forecaster-based approach with \rl in terms of generalization ability and sample-efficiency and show that the proposed approach can learn the system dynamics induced by user mobility with $100\times$ less training samples.

\textbf{Computationally efficient optimization algorithm.}
In \secref{sec:frank_wolfe_algo}, we propose an optimization algorithm to quickly solve the constrained utility maximization problem for user association.
We exploit the structure of the constraint set to derive an analytical solution for the direction-finding step in the projection-free Frank-Wolfe method.
Leveraging the analytically solution and backtracking line-search to dynamically adjust the step-size in every iteration, the execution time for solving the utility maximization can be reduced by two orders of magnitude compared to a generic convex solver.

\textbf{Realistic validation of rate gain and \ho reduction.}
In \secref{sec:results}, we evaluate the performance of the proposed forecaster-aided \mpc solution through extensive simulations using an industry-grade network simulator developed by Meta (formely Facebook) that accurately models a commercial cellular network.  We demonstrate that our \mpc approach can provide a more uniform user experience and improve the 5th percentile service rate by about $3.5\times$ compared to conventional strategies.
Furthermore, we show that by using our forecaster-based mobility-aware user association strategy, the median number of \hos in a time slot can be simultaneously reduced by about $7\times$ compared to a \ho agnostic strategy.


\textit{Notation}: $\bA_{:,i}$ denotes the $i$-th column of matrix $\bA$, $\bA_{i,:}$ denotes the $i$-th row of matrix $\bA$, $\bA^T$ denotes the transpose of a matrix, $[\bA]_{i,j}$ denotes the $(i,j)$-th element of $\bA$, and $\bA^\dagger$ denotes the Hermitian transpose of a matrix. The $i$-th element of vector $\ba$ is denoted by $a_i$. $\indicator{\cA}$ denotes the indicator function over set $\cA$, and $|\cA|$ denotes the cardinality of set $\cA$.

==> v2/system_model_GC.tex <==
\section{System Model}
\label{Sec:SysMod}

A downlink cellular network consisting of $K$ different frequency bands is considered. 
Let $\cB_k,~ k\in \{1, 2, \cdots, K\}$, denote the set of all base stations (BS) operating in the $k$-th frequency band and $\cU$ be the set of all UEs in the network. 
In this formulation, a BS is characterized by its physical deployment location \textit{and} the carrier frequency band used for transmissions. 
In other words, a physical site that supports two distinct frequency bands counts as two BSs, Fig. \ref{fig:network_struct}. 
It is easy to see that $\cB_k$ are disjoint sets and the set of all BSs can be denoted as $\cB = \bigcup_{k = 1}^K\cB_k$. 

The UEs are mobile and measure the received signal strength from their neighboring BSs, which can span multiple frequency bands, by measuring {\rm RSRP}s. 
\begin{figure}[t!]
    \centering
    \includegraphics[width=4in,                 keepaspectratio]{Figures/network_struct.pdf}
    \caption{Network structure and flow of RSRP and SINR measurements. The BSs receive RSRP measurement from the UEs in their cell. The central controller receives SINR measurements and load information from the BSs and communicates the association indicators back to the BSs and UEs.}
    \label{fig:network_struct}
\end{figure}
A slotted time model is considered where each UE reports the {\rm RSRP} from top-$m$ BSs to its serving BS, at the beginning of time slot $t$. For each UE $i$, the serving BS constructs the set $\{\mrsrp_{ij}[t]| j\in\cB\}$ by filling in zeros for the BSs for whom the measurements were not reported. 
Hence, $m$ should be large enough to include significant interferers. Given the RSRP measurements for a UE $i$, its SINR with BS $j\in \cB_k$ can be written as
\begin{align}
\label{eq:sinr_definition}
    \msinr_{ij}[t] &= \frac{\msnr{ij}[t]}{\sigma^2W_j + \sum_{j'\in \cB_k, j'\neq j}\msnr{ij'}[t]},
\end{align}
where $W_j$ represents the bandwidth of BS $j$ and $\sigma^2$ is the power spectral density of additive noise. 
Note that SINR is different from RSRP because it accounts for interference and depends on the bandwidth, whereas RSRP is a function of transmit power, pathloss, small scale fading, and large scale fading \cite[Section 8.1]{3GPP_36_873}. 
Let $\bm{\Phi}[t]$ denote the $|\cU|\times|\cB|$ matrix of SINRs such that $[\bm{\Phi}[t]]_{i,j} = \msinr_{ij}[t]$. 
$\ell_j[t]$ denote the load on BS $j$ (defined shortly), and $\bm{\ell}[t]$ be the vector of length $|\cB|$ representing the load on each BS in $\cB$. 
The BSs communicate their load and SINRs from their UEs to a central network controller in the RIC platform. 
The controller then decides the UE-BS association for the next time slot and communicates it to all the BSs, which then communicate it to the UEs. 
A HO event occurs if a UE changes its serving BS from one time slot to the next. 
Note that in this formulation HO occurs whenever the UE switches its band or site.

Since each BS generally serves more than one UE, its time and frequency resources need to be shared and the data rate for a UE depends on the load of the serving BS. The channel is assumed to be static during a time slot and all BSs are assumed to have full-buffers. The resources at each BS are distributed equally among the associated UEs, which is optimal in terms of log-utility achieved at each BS with static channels \cite{Ye13}. The data rate received by a UE $i$ associated to BS $j\in\cB_k$ can be expressed as
\begin{align}
    \label{eq:loaded_capacity_definition}
    c_{ij}[t] &= \frac{W_j}{\ell_j[t]}\log_2(1 + \msinr_{ij}[t]).
\end{align}
In case an HO is initiated, the UE's data transmission is interrupted for the related control signal exchange between the source and the target BSs \cite[Section 6]{3GPP_38_133}. Let $\tho{i}[t]$ be the HO interruption time experienced by UE $i$ during time slot $t$ and $T_s$ be the slot duration. The throughput for UE $i$ associated to BS $j\in\cB_k$, during time slot $t$, can be expressed as 
\begin{align}
    \label{eq:HO_capacity_definition}
    r_{ij}[t] &= \left(1 - \frac{\tho{i}[t]}{T_s}\right)c_{ij}[t]\\
                &= \left(1 - \frac{\tho{i}[t]}{T_s}\right)\frac{W_j}{\ell_j[t]}\log_2(1 + \msinr_{ij}[t]).
\end{align}
The following sections mathematically formulate the long-term utility maximization problem and the MDP for MLB.
